Learning Knowledge Bases with Parameters for Task-Oriented Dialogue Systems

Task-oriented dialogue systems are either modularized with separate dialogue state tracking (DST) and management steps or end-to-end trainable. In either case, the knowledge base (KB) plays an essential role in fulfilling user requests. Modularized systems rely on DST to interact with the KB, which is expensive in terms of annotation and inference time. End-to-end systems use the KB directly as input, but they cannot scale when the KB is larger than a few hundred entries. In this paper, we propose a method to embed the KB, of any size, directly into the model parameters. The resulting model does not require any DST or template responses, nor the KB as input, and it can dynamically update its KB via fine-tuning. We evaluate our solution in five task-oriented dialogue datasets with small, medium, and large KB size. Our experiments show that end-to-end models can effectively embed knowledge bases in their parameters and achieve competitive performance in all evaluated datasets.

==> img.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,328); %set diagram left start at 0, and has height of 328

%Shape: Circle [id:dp6462569817644479] 
\draw  [fill={rgb, 255:red, 204; green, 255; blue, 204 }  ,fill opacity=1 ] (404,138) .. controls (417.81,138) and (429,149.19) .. (429,163) .. controls (429,176.81) and (417.81,188) .. (404,188) .. controls (390.19,188) and (379,176.81) .. (379,163) .. controls (379,149.19) and (390.19,138) .. (404,138) -- cycle ;
%Shape: Circle [id:dp09829708114052349] 
\draw  [fill={rgb, 255:red, 255; green, 178; blue, 178 }  ,fill opacity=1 ] (404,8) .. controls (417.81,8) and (429,19.19) .. (429,33) .. controls (429,46.81) and (417.81,58) .. (404,58) .. controls (390.19,58) and (379,46.81) .. (379,33) .. controls (379,19.19) and (390.19,8) .. (404,8) -- cycle ;
%Shape: Circle [id:dp35709260739317195] 
\draw  [fill={rgb, 255:red, 255; green, 217; blue, 178 }  ,fill opacity=1 ] (404,268) .. controls (417.81,268) and (429,279.19) .. (429,293) .. controls (429,306.81) and (417.81,318) .. (404,318) .. controls (390.19,318) and (379,306.81) .. (379,293) .. controls (379,279.19) and (390.19,268) .. (404,268) -- cycle ;
%Shape: Circle [id:dp17761581355363965] 
\draw  [fill={rgb, 255:red, 255; green, 249; blue, 197 }  ,fill opacity=1 ] (274,138) .. controls (287.81,138) and (299,149.19) .. (299,163) .. controls (299,176.81) and (287.81,188) .. (274,188) .. controls (260.19,188) and (249,176.81) .. (249,163) .. controls (249,149.19) and (260.19,138) .. (274,138) -- cycle ;
%Shape: Circle [id:dp0036652641763266214] 
\draw  [fill={rgb, 255:red, 178; green, 178; blue, 255 }  ,fill opacity=1 ] (274,268) .. controls (287.81,268) and (299,279.19) .. (299,293) .. controls (299,306.81) and (287.81,318) .. (274,318) .. controls (260.19,318) and (249,306.81) .. (249,293) .. controls (249,279.19) and (260.19,268) .. (274,268) -- cycle ;
%Shape: Circle [id:dp1674491201227608] 
\draw  [fill={rgb, 255:red, 199; green, 239; blue, 252 }  ,fill opacity=1 ] (274,8) .. controls (287.81,8) and (299,19.19) .. (299,33) .. controls (299,46.81) and (287.81,58) .. (274,58) .. controls (260.19,58) and (249,46.81) .. (249,33) .. controls (249,19.19) and (260.19,8) .. (274,8) -- cycle ;
%Straight Lines [id:da06311645825500656] 
\draw    (404,58) -- (404,135) ;
\draw [shift={(404,138)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da9191872858106267] 
\draw    (379,33) -- (302,33) ;
\draw [shift={(299,33)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da19488975895282423] 
\draw    (404,268) -- (404,191) ;
\draw [shift={(404,188)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6119951335718659] 
\draw    (379,163) -- (302,163) ;
\draw [shift={(299,163)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da13367051606394753] 
\draw    (379,293) -- (302,293) ;
\draw [shift={(299,293)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6477505095556984] 
\draw    (274,268) -- (274,191) ;
\draw [shift={(274,188)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (388,260.2) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,rotate=-270] [align=left] {ActorsIn};
% Text Node
\draw (316.5,16.5) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {ActorsIn};
% Text Node
\draw (258,264) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,rotate=-270] [align=left] {HasGenre};
% Text Node
\draw (310,147) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {HasGenre};
% Text Node
\draw (388,121.2) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,rotate=-270] [align=left] {ActorsIn};
% Text Node
\draw (263.5,24.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {n2};
% Text Node
\draw (393.5,24.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {n1};
% Text Node
\draw (316.5,276.5) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {ActorsIn};
% Text Node
\draw (263.5,154.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {n5};
% Text Node
\draw (393.5,154.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {n3};
% Text Node
\draw (393.5,284.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {n4};
% Text Node
\draw (263.5,284.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {n6};


\end{tikzpicture}


==> main_img.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,385); %set diagram left start at 0, and has height of 385

%Rounded Rect [id:dp26286777867582733] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.6 ] (52,78.16) .. controls (52,75.31) and (54.31,73) .. (57.16,73) -- (138.89,73) .. controls (141.74,73) and (144.05,75.31) .. (144.05,78.16) -- (144.05,93.63) .. controls (144.05,96.48) and (141.74,98.79) .. (138.89,98.79) -- (57.16,98.79) .. controls (54.31,98.79) and (52,96.48) .. (52,93.63) -- cycle ;
%Rounded Rect [id:dp6259934910434752] 
\draw   (170.33,105.57) .. controls (170.33,102.03) and (173.2,99.17) .. (176.73,99.17) -- (210.27,99.17) .. controls (213.8,99.17) and (216.67,102.03) .. (216.67,105.57) -- (216.67,124.77) .. controls (216.67,128.3) and (213.8,131.17) .. (210.27,131.17) -- (176.73,131.17) .. controls (173.2,131.17) and (170.33,128.3) .. (170.33,124.77) -- cycle ;
%Rounded Rect [id:dp28937644596157996] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.6 ] (239,86.48) .. controls (239,84.56) and (240.56,83) .. (242.48,83) -- (318.42,83) .. controls (320.35,83) and (321.9,84.56) .. (321.9,86.48) -- (321.9,96.92) .. controls (321.9,98.85) and (320.35,100.4) .. (318.42,100.4) -- (242.48,100.4) .. controls (240.56,100.4) and (239,98.85) .. (239,96.92) -- cycle ;
%Rounded Rect [id:dp9593987165449438] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.6 ] (245,110.48) .. controls (245,108.56) and (246.56,107) .. (248.48,107) -- (307.76,107) .. controls (309.68,107) and (311.24,108.56) .. (311.24,110.48) -- (311.24,120.92) .. controls (311.24,122.85) and (309.68,124.4) .. (307.76,124.4) -- (248.48,124.4) .. controls (246.56,124.4) and (245,122.85) .. (245,120.92) -- cycle ;
%Rounded Rect [id:dp4498695909829886] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.6 ] (239,133.48) .. controls (239,131.56) and (240.56,130) .. (242.48,130) -- (315.76,130) .. controls (317.68,130) and (319.24,131.56) .. (319.24,133.48) -- (319.24,143.92) .. controls (319.24,145.85) and (317.68,147.4) .. (315.76,147.4) -- (242.48,147.4) .. controls (240.56,147.4) and (239,145.85) .. (239,143.92) -- cycle ;
%Curve Lines [id:da9307705272795086] 
\draw    (144.71,85.45) .. controls (166.71,87.07) and (154.05,115.74) .. (170.38,116.12) ;
%Curve Lines [id:da6814818366408693] 
\draw    (144.05,147.45) .. controls (167.38,148.12) and (151.71,117.45) .. (170.38,116.12) ;
%Straight Lines [id:da9651136954756039] 
\draw    (143.05,116.12) -- (170.38,116.12) ;
%Curve Lines [id:da8123928813185293] 
\draw    (216.38,115.45) .. controls (235.38,115.07) and (221.38,90.4) .. (238.38,91.45) ;
%Curve Lines [id:da8337817261399343] 
\draw    (216.38,115.45) .. controls (233.38,114.4) and (220.71,143.74) .. (239.05,139.45) ;
%Straight Lines [id:da029438912906568415] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  [dash pattern={on 4.5pt off 4.5pt}]  (48.05,167.93) -- (344.71,167.26) ;
%Flowchart: Magnetic Disk [id:dp8301220862670793] 
\draw   (194.33,29.22) -- (194.33,41.78) .. controls (194.33,43.65) and (189.11,45.17) .. (182.67,45.17) .. controls (176.22,45.17) and (171,43.65) .. (171,41.78) -- (171,29.22)(194.33,29.22) .. controls (194.33,31.09) and (189.11,32.6) .. (182.67,32.6) .. controls (176.22,32.6) and (171,31.09) .. (171,29.22) .. controls (171,27.35) and (176.22,25.83) .. (182.67,25.83) .. controls (189.11,25.83) and (194.33,27.35) .. (194.33,29.22) -- cycle ;
%Straight Lines [id:da5913830978406822] 
\draw    (94.05,51.98) -- (93.92,64.83) ;
\draw [shift={(93.9,66.83)}, rotate = 270.55] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Straight Lines [id:da5183367191838377] 
\draw    (160.71,50.6) -- (147.02,60.12) ;
\draw [shift={(145.38,61.26)}, rotate = 325.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Straight Lines [id:da036075877116884536] 
\draw    (215,36.5) -- (201.67,36.79) ;
\draw [shift={(199.67,36.83)}, rotate = 358.75] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-1.97) .. controls (4.17,-0.84) and (1.99,-0.18) .. (0,0) .. controls (1.99,0.18) and (4.17,0.84) .. (6.56,1.97)   ;
%Rounded Rect [id:dp9481062792326194] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.6 ] (52,108.16) .. controls (52,105.31) and (54.31,103) .. (57.16,103) -- (138.89,103) .. controls (141.74,103) and (144.05,105.31) .. (144.05,108.16) -- (144.05,123.63) .. controls (144.05,126.48) and (141.74,128.79) .. (138.89,128.79) -- (57.16,128.79) .. controls (54.31,128.79) and (52,126.48) .. (52,123.63) -- cycle ;
%Rounded Rect [id:dp6013466224907857] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.6 ] (52,138.16) .. controls (52,135.31) and (54.31,133) .. (57.16,133) -- (138.89,133) .. controls (141.74,133) and (144.05,135.31) .. (144.05,138.16) -- (144.05,153.63) .. controls (144.05,156.48) and (141.74,158.79) .. (138.89,158.79) -- (57.16,158.79) .. controls (54.31,158.79) and (52,156.48) .. (52,153.63) -- cycle ;
%Straight Lines [id:da38493466519559827] 
\draw    (217.05,115.12) -- (244.38,115.12) ;
%Rounded Rect [id:dp9257586521562136] 
\draw   (170.33,185.57) .. controls (170.33,182.03) and (173.2,179.17) .. (176.73,179.17) -- (210.27,179.17) .. controls (213.8,179.17) and (216.67,182.03) .. (216.67,185.57) -- (216.67,204.77) .. controls (216.67,208.3) and (213.8,211.17) .. (210.27,211.17) -- (176.73,211.17) .. controls (173.2,211.17) and (170.33,208.3) .. (170.33,204.77) -- cycle ;
%Rounded Rect [id:dp7771622324925265] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.6 ] (245,190.48) .. controls (245,188.56) and (246.56,187) .. (248.48,187) -- (307.76,187) .. controls (309.68,187) and (311.24,188.56) .. (311.24,190.48) -- (311.24,200.92) .. controls (311.24,202.85) and (309.68,204.4) .. (307.76,204.4) -- (248.48,204.4) .. controls (246.56,204.4) and (245,202.85) .. (245,200.92) -- cycle ;
%Straight Lines [id:da5795415334111893] 
\draw    (143.05,196.12) -- (170.38,196.12) ;
%Rounded Rect [id:dp6325870693433393] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.6 ] (52,188.16) .. controls (52,185.31) and (54.31,183) .. (57.16,183) -- (138.89,183) .. controls (141.74,183) and (144.05,185.31) .. (144.05,188.16) -- (144.05,203.63) .. controls (144.05,206.48) and (141.74,208.79) .. (138.89,208.79) -- (57.16,208.79) .. controls (54.31,208.79) and (52,206.48) .. (52,203.63) -- cycle ;
%Straight Lines [id:da7047925599631482] 
\draw    (217.05,195.12) -- (244.38,195.12) ;

% Text Node
\draw (54.48,74) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont Is there any resturant}}\\{\tiny {\fontfamily{pcr}\selectfont that servers Italian food?}}};
% Text Node
\draw (171.33,104.57) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {{\fontfamily{pcr}\selectfont GPT-2}};
% Text Node
\draw (239.69,88) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {\scalebox{.7}{ {\fontfamily{pcr}\selectfont There is Pizza Express.}}};
% Text Node
\draw (245.69,107) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont There is Kohinoor.}}};
% Text Node
\draw (242.48,130) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont There is Golden Wok.}}};
% Text Node
\draw (218.35,27.33) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont SELECT type,name FROM Resturant}}};
% Text Node
\draw (45.02,20.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont USR: Is there any resturant }}\\{\tiny {\fontfamily{pcr}\selectfont  \ \ \ \ \ \ \ that servers <type> food?}}\\{\tiny {\fontfamily{pcr}\selectfont SYS: There is <name>}}};
% Text Node
\draw (174.67,24.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny {\fontfamily{pcr}\selectfont KB}}};
% Text Node
\draw (53.48,104) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont Is there any resturant}}\\{\tiny {\fontfamily{pcr}\selectfont that servers Chinese food?}}};
% Text Node
\draw (53.48,134) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont Is there any resturant}}\\{\tiny {\fontfamily{pcr}\selectfont that servers Indian food?}}};
% Text Node
\draw (171.33,184.57) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {{\fontfamily{pcr}\selectfont GPT-2}};
% Text Node
\draw (246.69,187) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont There is Kohinoor.}}};
% Text Node
\draw (53.48,184) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {{\tiny {\fontfamily{pcr}\selectfont I would like a resturant}}\\{\tiny {\fontfamily{pcr}\selectfont with Indian food?}}};


\end{tikzpicture}

